Efficiently Disentangle Causal Representations

This paper proposes an efficient approach to learning disentangled representations with causal mechanisms based on the difference of conditional probabilities in original and new distributions. We approximate the difference with models' generalization abilities so that it fits in the standard machine learning framework and can be efficiently computed. In contrast to the state-of-the-art approach, which relies on the learner's adaptation speed to new distribution, the proposed approach only requires evaluating the model's generalization ability. We provide a theoretical explanation for the advantage of the proposed method, and our experiments show that the proposed technique is 1.9--11.0$\times$ more sample efficient and 9.4--32.4 times quicker than the previous method on various tasks. The source code is available at \url{https://github.com/yuanpeng16/EDCR}.

==> abstract_modified.tex <==
Causal representation is important aspect of artificial intelligence and receiving increasing attentions.
In this paper, we show that disentangling causal representations can be more efficient by leveraging model's generalization ability.
%
%In this paper, w
We propose a novel approach to efficiently learning disentangled representations with causal mechanisms, based on the difference of conditional probabilities in original and new distributions.
We approximate the difference with model's generalization abilities so that it fits in standard machine learning framework and can be efficiently computed.
In contrast to the state-of-the-art approach, which relies on learner's adaptation speed to new distribution, the proposed approach only requires evaluating the generalization ability of the model.
We provide theoretical explanation for the advantage of the proposed method, and our experiments show that the proposed technique is 1.9--11.0$\times$ more sample efficient and 9.4--32.4$\times$ quicker than the previous method on various tasks.
The source code is in supplementary material.


==> intro.tex <==
Causal reasoning is a fundamental  tool that has shown great impact in different disciplines~\citep{rubin2006estimating,ramsey2010six,rotmensch2017learning}, and it has roots in work by David Hume in the eighteenth century~\citep{hume2003treatise} and in classical AI~\citep{pearl2003causality}. Causality has been mainly studied from a statistical perspective~\citep{greenland1999causal,pearl2009causality,pearl2018does} with Judea Pearl's work on the causal calculus leading its statistical development.

More recently, there has been a growing interest to integrate statistical techniques into machine learning to leverage their benefits.
Welling raises a particular question about how to disentangle correlation from causation in machine learning settings to take advantage of the sample efficiency and generalization abilities of causal reasoning~\citep{welling2015ml}.
Although machine learning has achieved important results on a variety of tasks like computer vision and games over the past decade (e.g., \cite{mnih2015human,silver2017mastering,szegedy2017inception,hudson2018compositional}), current approaches can struggle to generalize when the test data distribution is much different from the training distribution (common in real applications). Further, these successful methods are typically ``data hungry'', requiring an abundance of labeled examples to perform well across data distributions.

In statistical settings, encoding the causal structure in models has been shown to have significant efficiency advantages.
For example, in the context of speech recognition, \cite{chorowski2014end} and \cite{Bengio17} show that a model trained to learn $P(\text{acoustics})$ performs worse than a model trained to also learn a conditional distribution containing phonemes, $P(\text{acoustics}|\text{phonemes}) \cdot P(\text{phonemes})$. The model performs better when the causality---phonemes cause acoustics---is encoded in the model.
Further, \cite{scholkopf2012causal} show that encoding the causal structure leads to more robust estimation (and thus, the performance improves).
Independent of any change in $P(\text{phonemes})$, the causal mechanism $P(\text{acoustics}|\text{phonemes})$ is not expected to change across tasks or datasets. These robustness and generalization characteristics lead to quicker training, because once the causal mechanism is learned, it requires minimal updates to transfer to new data.

In support of the advantages of encoding causal mechanisms, \cite{bengio2020a} recently introduced an approach to disentangling causal relationships in end-to-end machine learning by comparing the adaptation speeds of separate models that encode different causal structures.
The core idea is explained with an atmospheric physics example of learning $P(A,B)$, where $A$ (\textbf{Altitude}) causes $B$ (\textbf{Temperature})~\citep{peters2016causal}. The marginal probability of $A$ can be changed depending on, for instance, the place (Switzerland to less mountainous country like Netherlands), but $P(B|A)$ as the underlining causality mechanism does not change. Therefore, the causality structure can be inferred from the robustness of predictive models on out-of-distribution~\citep{peters2016causal,peters2017elements}.
The invariance of $P(B|A)$ across train and transfer distributions is the key assumption in their work, and we also follow it in this work.

$P(A,B)$ can be either modeled as $P(B|A) \cdot P(A)$ or $P(A|B) \cdot P(B)$, reflecting the possible causal directions. Since $P(B|A) \cdot P(A)$ reflects the right causal structure, it is more efficient to adapt to a change in $P(A)$ since parameters for $P(B|A)$ need not to be updated. On the other hand, the model that assumes the opposite causal direction, $P(A|B) \cdot P(B)$, must adapt both its marginal and conditional distribution parameters, leading to slower adaptation speed.
The previous method proposed the state-of-the-art meta-learning approach to disentangling causal mechanisms using the adaptation speed as a meta-objective to optimize. In particular, the task is to determine whether the causal direction is $A\rightarrow B$ or $B \rightarrow A$.


\emph{In this work}, we propose a more efficient approach to disentangling causal mechanisms than the state-of-the art one based on the same assumption.
The baseline approach essentially captures the changes in $P(B|A)$ and $P(A|B)$, by examining how fast the joint probability models can adapt or learn after intervention.
In contrast, our approach only evaluates the generalization ability of the model without the need of the adaptation process, therefore it is much quicker in disentangling the causal mechanisms.
Our experiments show the proposed technique is 1.9--11.0$\times$ more sample efficient and 9.4--32.4$\times$ quicker than measuring adaptation speed on various tasks.
We also argue that the proposed approach has less hyper parameters and it is straight-forward to implement the approach within the standard machine learning workflows.

Our contributions can be summarized as follows.
\begin{itemize}
    \item We propose an efficient approach to disentangling representations for causal mechanisms by measuring generalization.
    \item We theoretically prove that the proposed estimators can identify
    causal direction and disentangles causal mechanisms.
    %\item We provide proofs for using conditional KL-divergence to detect causality direction and for generalization loss closely approximating divergence.
    \item We empirically show that the proposed approach is significantly quicker and more sample efficient for various tasks. Sample efficiency is important when data size in transfer distribution is small.
    
    %The source code is included in supplementary material, and will be publicly available upon acceptance.
\end{itemize}

